Dynamically Iterated Filters: A unified framework for improved iterated filtering and smoothing

Typical iterated filters, such as the iterated extended Kalman filter (IEKF), iterated unscented Kalman filter (IUKF), and iterated posterior linearization filter (IPLF), have been developed to improve the linearization point (or density) of the likelihood linearization in the well-known extended Kalman filter (EKF) and unscented Kalman filter (UKF). A shortcoming of typical iterated filters is that they do not treat the linearization of the transition model of the system. To remedy this shortcoming, we introduce dynamically iterated filters (DIFs), a unified framework for iterated linearization-based nonlinear filters that deals with nonlinearities in both the transition model and the likelihood, thereby constituting a generalization of the aforementioned iterated filters. We further establish a relationship between the general DIF and the approximate iterated Rauch-Tung-Striebel smoother. This relationship allows for a Gauss-Newton interpretation, which in turn enables explicit step-size correction, leading to damped versions of the DIFs. The developed algorithms, both damped and non-damped, are numerically demonstrated in three examples, showing superior mean-squared error as well as improved parameter tuning robustness as compared to the analogous standard iterated filters.

==> sections/background.tex <==
For clarity, we here present analytical and statistical linearization in a common framework, as well as restate the well-known \gls{ks} equations.

\subsection{(Affine) Kalman Smoother}
The well--known \gls{kf} and \abbrRTS smoother equations are repeated here for clarity in terms of a time update, measurement update, and a smoothing step. These can for instance be found in \cite{sarkkaBayesianFilteringSmoothing2013}.
Assume an affine state--space model with additive Gaussian noise, such as
\begin{subequations}
\begin{align}
\state_{k+1} &= \vec{A}_\dynmod\state_k + \vec{b}_\dynmod + \tilde{\pnoise}_k\\
\obs_k &= \vec{A}_\obsmod\state_k + \vec{b}_\obsmod + \tilde{\onoise}_k.
\end{align}
\end{subequations}
Here,  $\tilde{\pnoise}_k\sim\Ndist(\tilde{\pnoise}_k;\vec{0},\vec{Q}\!+\!\boldsymbol{\Omega}_\dynmod)$ and $\tilde{\onoise}_k\sim\Ndist(\tilde{\onoise}_k;\vec{0},\vec{R}\!+\!\boldsymbol{\Omega}_\obsmod)$ are assumed to be mutually independent.
Note that usually, $\boldsymbol{\Omega}_\dynmod=\boldsymbol{\Omega}_\obsmod=\vec{0}$.
For this model, the (affine) \gls{ks} update equations are given by \cref{alg:kalmansmoother}.
\begin{algorithm}[tb]
\caption{(Affine) Kalman smoother}
\label{alg:kalmansmoother}
\begin{enumerate}
\item Time update
\begin{subequations}
\label{eq:timeupdate}
\begin{align}
\hspace*{\dimexpr-\leftmargini}\hat{\state}_{k+1|k} &= \vec{A}_\dynmod\hat{\state}_{k|k} + \vec{b}_\dynmod\\
\hspace*{\dimexpr-\leftmargini}\vec{P}_{k+1|k} &= \vec{A}_\dynmod\vec{P}_{k|k}\vec{A}_\dynmod^\top + \vec{Q} + \boldsymbol{\Omega}_\dynmod.
\end{align}
\end{subequations}
\item Measurement update
\begin{subequations}
\label{eq:measupdate}
\begin{align}
\hspace*{\dimexpr-\leftmargini}\hat{\state}_{k|k} &= \hat{\state}_{k|k-1} + \vec{K}_k(\obs_k - \vec{A}_\obsmod\hat{\state}_{k|k-1} - \vec{b}_\obsmod)\\
\hspace*{\dimexpr-\leftmargini}\vec{P}_{k|k} &= \vec{P}_{k|k-1} - \vec{K}_k\vec{A}_\obsmod\vec{P}_{k|k-1}\\
\hspace*{\dimexpr-\leftmargini}
\vec{K}_k &\triangleq \vec{P}_{k|k-1}\vec{A}_\obsmod^\top(\vec{A}_\obsmod\vec{P}_{k|k-1}\vec{A}_\obsmod^\top + \vec{R} + \boldsymbol{\Omega}_\obsmod)^{-1}.
\end{align}
\end{subequations}
\item Smoothing step
\begin{subequations}
\label{eq:smoothstep}
\begin{flalign}
\hspace*{\dimexpr-\leftmargini}\hat{\state}_{k|K} &= \hat{\state}_{k|k} + \vec{G}_k (\hat{\state}_{k+1|K} - \hat{\state}_{k+1|k})\\
\hspace*{\dimexpr-\leftmargini}\vec{P}_{k|K} &= \vec{P}_{k|k} + \vec{G}_k(\vec{P} _{k+1|K} -\nonumber\\ &\quad~ \vec{A}_\dynmod\vec{P}_{k|k}\vec{A}_\dynmod^\top-\vec{Q}-\boldsymbol{\Omega}_\dynmod)\vec{G}_k^\top\\
\hspace*{\dimexpr-\leftmargini}\vec{G}_k &\triangleq  \vec{P}_{k|k}\vec{A}_\dynmod^\top(\vec{A}_\dynmod\vec{P}_{k|k}\vec{A}_\dynmod^\top + \vec{Q} + \boldsymbol{\Omega}_\dynmod)^{-1}
\end{flalign}
\end{subequations}
\end{enumerate}
\end{algorithm}

\subsection{Analytical and Statistical Linearization}
Given a nonlinear model
\begin{equation*}
\vec{z} = \vec{g}(\state),
\end{equation*}
we wish to find an affine representation
\begin{equation}
\vec{g}(\state)\approx \vec{A}\state + \vec{b} + \eta,
\end{equation}
with $\eta\sim\Ndist(\eta; \vec{0}, \boldsymbol{\Omega})$.
In this affine representation, there are three free parameters: $\vec{A}, \vec{b}$ and $\boldsymbol{\Omega}$.
Analytical linearization, through first--order Taylor expansion, selects the parameters as
\begin{equation}\label{eq:analyticallinearization}
\vec{A}=\frac{d}{d\state}\vec{g}(\state)|_{\state=\bar{\state}},
\quad \vec{b} = \vec{g}(\state)|_{\state=\bar{\state}} - \vec{A}\bar{\state},
\quad \boldsymbol{\Omega}=\vec{0},
\end{equation}
where $\bar{\state}$ is the point about which the function $\vec{g}(\state)$ is linearized.
Note that $\boldsymbol{\Omega}=\vec{0}$ essentially implies that the linearization is assumed to be error free.

Statistical linearization instead linearizes w.r.t. a distribution $p(\state)$.
Practically, one may think of this as constructing an affine function that best fits a number of samples of $p(\state)$ transformed through $\vec{g}(\state)$.
Assuming that such a distribution $p(\state)=\Ndist(\state;\hat{\state},\vec{P})$ is given, statistical linearization selects the affine parameters as
\begin{subequations}\label{eq:statisticallinearization}
\begin{align}
\vec{A} &= \Psi^\top \vec{P}^{-1}\\
\vec{b} &= \bar{\vec{z}}-\vec{A}\hat{\state}\\
\boldsymbol{\Omega} &= \Phi-\vec{A} \vec{P} \vec{A}^\top\\
%
\bar{\vec{z}} &= \mathbb{E}[\vec{g}(\state)]\\
%
\Psi &= \mathbb{E}[(\state-\hat{\state})(\vec{g}(\state) - \bar{\vec{z}})^\top]\\
%
\Phi &= \mathbb{E}[(\vec{g}(\state) - \bar{\vec{z}})(\vec{g}(\state) - \bar{\vec{z}})^\top],
\end{align}
\end{subequations}
where the expectations are taken w.r.t. $p(\state)$.
The major difference from analytical linearization is that typically ${\boldsymbol{\Omega}\neq 0}$, implying that the error in the linearization is captured.
Typically, the expectations in \cref{eq:statisticallinearization} are not analytically tractable and thus, practically, one often resorts to some numerical integration technique.

==> sections/fig1_tikz.tex <==
\begin{tikzpicture}[squarednode/.style={rectangle, draw=black, text opacity=1, thick, minimum size=5mm},
every node/.style={inner sep=5pt,outer sep=0pt, font=\footnotesize}]
\node (in) {$q(\state_{k-1}|\obs_{1:k-1})$};

% Time
\node[squarednode] (timeupdate) [right=of in, xshift=1cm] {TU};
% In to time
\draw[-latex, thick] (in.east) -- (timeupdate.west);

% Meas
\node[squarednode] (measupdate) [right=of timeupdate, xshift=1.5cm] {MU};
% Meas to out
\draw[-latex, thick] (measupdate.east) -- ++(2.0, 0) node[label=right:{$q^i(\state_{k}|\obs_{1:k})$}] {};
% Meas to meas
\draw[-latex, thick] ($(measupdate.east)+(1.0, 0)$) -- ++(0, 1.) node[label=above:{Lin. point}, yshift=-.25cm, xshift=-.5cm] {} -| (measupdate.north);

% Smooth
\node[squarednode] (smoothing) [below=of measupdate, yshift=-.5cm] {S};
% Time to meas
\draw[-latex, thick] (timeupdate.east) -- node[label={[text=snsblue]above:{$q^i(\state_{k}|\obs_{1:k-1})$}}, yshift=-.1cm] {} (measupdate.west);
% Meas to smooth
\draw[-latex, thick] ($(measupdate.east)+(1.0, 0)$) |- (smoothing.east);
% Smooth to time
\draw[-latex, thick] (smoothing.west) -| node[label={[text=snsblue]left:{$q^i(\state_{k-1}|\obs_{1:k})$}}, yshift=.5cm] {} node[yshift=-.25cm, label=above:{Lin. point}, xshift=1.cm] {} (timeupdate.south);
% Smooth to smooth
\draw[-latex, thick] ($(smoothing.west)+(-1.25, 0)$) -- ++(0, .75) node[label=above:{Lin. point}, yshift=-.25cm, xshift=.75cm] {} -| (smoothing.north);

% Iterated filters box
\draw[ultra thick, dotted, snsorange] (measupdate.north west)+(-.25, 1.25)
node [xshift=2.cm, yshift=-.2cm, label=above:{Iterated Filters}] {}
rectangle ($(measupdate.south east)+(2, -0.25)$);
% Dynamically Iterated filters box
\draw[ultra thick, dotted, snsblue] (timeupdate.north west)+(-2, 1.25)
node [xshift=1.75cm, yshift=-4cm, label=below:{Dynamically Iterated Filters}] (DIF) {}
rectangle ($(smoothing.south east)+(2.165, -0.1)$);
\end{tikzpicture}

==> sections/solution.tex <==
In order to derive an algorithm encompassing both the transition density \cref{eq:transdensityapprox} as well as the observation density \cref{eq:obsdensityapprox} at time $k$, we naturally need to seek an approximate posterior over both $\state_{k-1}$ as well as $\state_k$.
In order to do so, we generalize the derivation in \cite{garcia-fernandezPosteriorLinearizationFilter2015} to extend backwards one step.
Define two auxiliary variables, $\auxil_k,~\auxil_{k-1}$ as
\begin{subequations}
\begin{align}
\auxil_{k-1} &= \dynmod(\state_{k-1}) + \psi\\
\auxil_k &= \obsmod(\state_k) + \phi\\
p(\psi) &= \Ndist(\vec{0}, \alpha\vec{I}),\quad
p(\phi) = \Ndist(\vec{0}, \beta\vec{I}),
\end{align}
\end{subequations}
where $\psi$ and $\phi$ are independent of each other as well as the process noise $\pnoise$ and the measurement noise $\onoise$.
Note that as $\alpha,~\beta\to 0$, $\auxil_{k-1}\to \dynmod(\state_{k-1})$ and $\auxil_k\to\obsmod(\state_k)$.
Now, the true joint posterior of $\state_{k-1},~\state_k,~\auxil_{k-1}$ and $\auxil_k$ is given by
\begin{align}\label{eq:jointdecomposition}
&\fulljoint \propto\nonumber \\&\fulljointexpand.
\end{align}
Following \cite{garcia-fernandezPosteriorLinearizationFilter2015}, we assume that the approximate posterior decomposes in the same manner, i.e.,
\begin{align}\label{eq:approximatejoint}
 &\approxjoint \approx \nonumber\\&\approxjointexpand,
\end{align}
where $\theta$ are the parameters of the affine approximation of the transition model and measurement model, i.e., ${\theta=[\vec{A}_\dynmod,\vec{b}_\dynmod,\boldsymbol{\Omega}_\dynmod, \vec{A}_\obsmod,\vec{b}_\obsmod,\boldsymbol{\Omega}_\obsmod]}$.

We can now compute the Kullback-Leibler (\abbrKL) divergence between the true joint posterior and the approximation as
\begin{align}
&\mathrm{KL}\left(\fulljoint \Vert \approxjoint \right)\nonumber=\\
&\mathrm{KL}\left( \statejoint \Vert \approxstatejoint \right) +\nonumber\\
&\mathbb{E}\left[\mathrm{KL}(\auxilcond{k}\Vert\approxauxilcond{k})\right] +\nonumber\\
&\mathbb{E}\left[
\mathrm{KL}(\auxilcond{k-1}\Vert\approxauxilcond{k-1})
\right] \triangleq\Loss, \label{eq:fulloss}
\end{align}
see \cref{app:loss} for the derivation.
Note that the expectations in $\Loss$ are taken with respect to the true joint posterior $\statejoint$.
It is noteworthy that $\Loss$ decomposes into three distinct terms, each dealing with each respective factor of \cref{eq:approximatejoint}.
The first term is simply the \abbrKL divergence between the true and approximate joint posterior of the states at time $k$ and $k-1$.
The second and third terms are the expected \abbrKL divergences of the affine approximation of the measurement model and transition model, respectively, where the expectation is taken with respect to the true joint posterior $\statejoint$.

The optimal affine approximations of $\dynmod$ and $\obsmod$ are thus given by
\begin{align}\label{eq:fullopt}
\theta^* = &\arg\min_\theta \Loss,
\end{align}
where $\Loss$ is given by \cref{eq:fulloss}.
However, it is impractical to minimize \cref{eq:fulloss}, seeing as it requires knowledge of the true joint posterior $\statejoint$.
Nevertheless, an iterative procedure may be used to approximately solve this minimization problem.
% Seeing as the first term of $\Loss$ is $\geq 0$, a lower bound is given by the second term, i.e.,
% \begin{equation*}
% \Loss \geq \mathbb{E}
% \left[
% \mathrm{KL}(\auxilcond{k}\Vert\approxauxilcond{k}) + \mathrm{KL}(\auxilcond{k-1}\Vert\approxauxilcond{k-1})
% \right].
% \end{equation*}
% Hence, the optimal linear approximations of $f$ and $h$ are given by
% \begin{equation*}
% \theta^* = \arg\min_\theta \mathbb{E}_{\statejoint}
% \left[
% \mathrm{KL}(\auxilcond{k}\Vert\approxauxilcond{k}) + \mathrm{KL}(\auxilcond{k-1}\Vert\approxauxilcond{k-1})
% \right],
% \end{equation*}
% where $\theta$ includes all the parameters of the linearization(s).

\subsection{Iterative Solution}
To practically optimize \cref{eq:fullopt}, assume access to an $i$:th approximation to the state joint posterior $\statejoint\approx\approxstatejoint[i]$ and replace all occurences of $\statejoint$ in $\Loss$ with this approximation.
The optimization problem \cref{eq:fullopt} then turns into
\begin{align*}
\theta^* = &\arg\min_{\theta}
\mathrm{KL}\left( \approxstatejoint[i] \Vert \approxstatejoint[i+1] \right) +\nonumber\\
&\mathbb{E}_{\approxstatejoint[i]}\left[\mathrm{KL}(\auxilcond{k}\Vert\approxauxilcond[i+1]{k})\right] +\nonumber\\
&\mathbb{E}_{\approxstatejoint[i]}
\left[
\mathrm{KL}(\auxilcond{k-1}\Vert\approxauxilcond[i+1]{k-1})
\right],
\end{align*}
where the expectations are now over $\approxstatejoint[i]$ instead.
Sufficiently close to a fixed point, the first \abbrKL term is approximately 0 and the final optimization problem is thus given by
\begin{align}
\theta^* = &\arg\min_{\theta}
\mathbb{E}_{\approxstatejoint[i]}\biggl[\mathrm{KL}(\auxilcond{k}\Vert\approxauxilcond[i+1]{k}) +\nonumber\\
&\mathrm{KL}(\auxilcond{k-1}\Vert\approxauxilcond[i+1]{k-1})
\biggr].
\end{align}
Technically, the optimal $\theta^*$ is given by statistical linearization of $\dynmod$ and $\obsmod$ w.r.t. the current approximation $\approxstatejoint[i]$, see e.g. \cite{garcia-fernandezPosteriorLinearizationFilter2015}.
Note that statistical linearization of $\dynmod$ w.r.t. $\approxstatejoint[i]$ only requires the marginal $\approxstate{i}{k-1}$.
Similarly, statistical linearization of $\obsmod$ only requires the marginal $\approxstate{i}{k}$.
Thus, the algorithm conceptually amounts to predicting forward in time, performing a measurement update and smoothing backwards in time in order to provide new linearization points (densities) for both the transition density as well as the measurement density simultaneously.
These steps are then iterated until convergence, finally providing an approximate posterior $q(\state_k|\obs_{1:k})$.
The general algorithm is summarized in \cref{alg:dyniterfilter} and schematically depicted in \cref{fig:dyniterfilter}.

% Schematic illustration of a dynamically iterated filter
\begin{figure}[tb]
\centering
\begin{tikzpicture}[squarednode/.style={rectangle, draw=black, text opacity=1, thick, minimum size=5mm},
every node/.style={inner sep=5pt,outer sep=0pt, font=\footnotesize}]
\node[squarednode] (previous) {$q(\state_{k-1}|\obs_{1:k-1})$};
\node[squarednode] (predicted) [right=of previous] {$q(\state_{k}|\obs_{1:k-1})$};
\node[squarednode] (updated) [right=of predicted] {$q(\state_{k}|\obs_{1:k})$};
\node[squarednode, draw=snsblue, text=snsblue] (smoothed) [below=of predicted] {$q(\state_{k-1}|\obs_{1:k})$};
% Prediction step
\draw[-latex, thick] (previous.east) -- node[inner sep=0pt, label=above:{TU}] (timeupdate) {} (predicted.west);
% Update step
\draw[-latex, thick] (predicted.east) -- node[label=below:{MU}, inner sep=0pt] (measurementupdate) {} (updated.west);
% Smoothing step
\draw[-latex, thick, snsblue] (updated.south) |-  node[inner sep=0pt, xshift=-.75cm, label=above:{S}] (smoothstep) {} (smoothed.east);
% Prediction re-linearization
\draw[-latex, thick, snsblue] (smoothed.west) -| node[label=left:{Re-linearize}, yshift=.6cm, xshift=.25cm] {} (timeupdate.south);
% Update re-linearization
\draw[-latex, thick] (updated.north) |- ++(0, 0.25) -| node[label=above:{Re-linearize}, xshift=.6cm, yshift=-.25cm] {} (measurementupdate.north);
% Smoothing re-linearization
\draw[-latex, thick, snsblue] (smoothed.south) |- ++(0, -0.25) node[xshift=1cm, yshift=.25cm, label=below:{Re-linearize}] {} -| (smoothstep.south);
% Rectangle around update step
\draw[ultra thick, dotted, snsred] (updated.north west)+(-.85, .75)
node [xshift=1.5cm, yshift=-.25cm, label=above:{Iterated Filters}] {}
rectangle ($(updated.south east)+(0.25, -0.25)$);
\end{tikzpicture}
\caption{Schematic illustration of a dynamically iterated filter. Ordinary iterated filters, marked in dotted red, only re-linearize the measurement update. Dynamically iterated filters also re-linearize the time update through a smoothing step, marked in blue. The time update (TU) and the smoothing step (S) are linearized w.r.t. the smoothed distribution $q(\state_{k-1}|\obs_{1:k})$. The measurement update (MU) is linearized w.r.t. the current posterior $q(\state_k|\obs_{1:k})$. The steps are iterated until some convergence criterion is met.}
\label{fig:dyniterfilter}
\end{figure}

% An algorithmic description of a dynamically iterated filter
\begin{algorithm}
\caption{A dynamically iterated filter}
\label{alg:dyniterfilter}
\begin{algorithmic}
\Require $q(\state_{k-1}|\obs_{1:k-1})=\Ndist(\state_{k-1};\hat{\state}_{k-1|k-1},\vec{P}_{k-1|k-1})$
\State Compute $\hat{\state}_{k|k-1}^0, \vec{P}_{k|k-1}^0$ by \cref{eq:timeupdate}
\State Compute $\hat{\state}_{k|k}^0, \vec{P}_{k|k}^0$ by \cref{eq:measupdate}
\State Compute $\hat{\state}_{k-1|k}^0, \vec{P}_{k-1|k}^0$ by \cref{eq:smoothstep}
\State $i\gets 0$
\While{not converged}
  \State Calculate $(\vec{A}_\dynmod,\vec{b}_\dynmod, \boldsymbol{\Omega}_\dynmod)$ by analytical or statistical linearization of $\dynmod$ about $\hat{\state}_{k-1|k}^i, \vec{P}_{k-1|k}^i$
  \State Compute $\hat{\state}_{k|k-1}^{i+1}, \vec{P}_{k|k-1}^{i+1}$ by \cref{eq:timeupdate}
  \State Calculate $(\vec{A}_\obsmod,\vec{b}_\obsmod, \boldsymbol{\Omega}_\obsmod)$ by analytical or statistical linearization of $\obsmod$ about $\hat{\state}_{k|k}^i, \vec{P}_{k|k}^i$
  \State Compute $\hat{\state}_{k|k}^{i+1}, \vec{P}_{k|k}^{i+1}$ by \cref{eq:measupdate}
  \State Compute $\hat{\state}_{k-1|k}^{i+1}, \vec{P}_{k-1|k}^{i+1}$ by \cref{eq:smoothstep}
  \State $i\gets i+1$
\EndWhile
\State \textbf{return} $\hat{\state}_{k|k}^{i}, \vec{P}_{k|k}^{i}$
\end{algorithmic}
\end{algorithm}

Note that the algorithm is applicable to all possible combinations of models with linear and nonlinear $\dynmod$ and $\obsmod$.
Further, even though the developed solution is essentially an \abbrIPLF also encompassing the transition density, by changing the linearization method from statistical to analytical, an ``extended'' version is recovered in similar spirit to the \abbrIEKF.
Furthermore, an \abbrIUKF version, similar to \cite{skoglundIterativeUnscentedKalman2019}, may also be recovered by ``freezing'' the covariance matrices $\vec{P}_{k-1|k}^i=\vec{P}_{k-1|k-1}$ and $\vec{P}_{k|k}^i=\vec{P}^i_{k|k-1}$ and only updating these during the last iteration.
It is also worthwhile to point out that the dynamically iterated filters are essentially ``local'' iterated smoothers, analogous to the \emph{iterated extended Kalman smoother} (\abbrIEKS) \cite{bellIteratedKalmanSmoother1994a} and the \emph{iterated posterior linearization smoother} (\abbrIPLS) \cite{garcia-fernandezIteratedPosteriorLinearization2017}, operating on just one time instance and observation.
Therefore, as noted in \cite{raitoharjuPosteriorLinearisationFilter2022}, a byproduct of the algorithm is a one-step smoothed state estimate and the method can thus be thought of as an iterated one-step fixed-lag smoother as well.

All that is left is to determine a stopping criterion for the iterations.
Similarly to \cite{garcia-fernandezPosteriorLinearizationFilter2015}, a stopping criterion for the iterative updates may be formed on the basis of the \abbrKL divergence between two successive approximations of the posterior, i.e.,
\begin{equation*}
\mathrm{KL}(q^i(\state_k|\obs_{1:k})\Vert q^{i+1}(\state_k|\obs_{1:k})) < \gamma.
\end{equation*}
Another possibility to check for fixed-point convergence is to instead use the smoothed density $q(\state_{k-1}|\obs_{1:k})$ in a similar manner as the posterior.
This is not investigated in detail here.
Instead, in the numerical example in \cref{sec:examples}, a fixed number of iterations is used for simplicity.

% \subsection{Stopping Criterion}
% Similarly to \cite{garcia-fernandezPosteriorLinearizationFilter2015}, a stopping criterion for the iterative updates may be formed on the basis of the \abbrKL divergence between two successive approximations of the posterior.
% However, in the dynamically iterated filters proposed here, there are two densities that may be used for checking fixed-point convergence: the posterior $q(\state_k|\obs_{1:k})$ as well as the smoothed density $q(\state_{k-1}|\obs_{1:k})$.
% Our interest in this particular paper is still to improve the posterior approximation and we therefore propose to use the same criterion as \cite{garcia-fernandezPosteriorLinearizationFilter2015}, i.e.,
% \begin{equation}
% \mathrm{KL}(q^i(\state_k|\obs_{1:k})\Vert q^{i+1}(\state_k|\obs_{1:k})) < \gamma.
% \end{equation}
% Hence, the iterations are stopped if the \abbrKL divergence between two successive approximate posteriors is below $\gamma$.

\subsection{Illustrative example}
In order to illustrate the iterative procedure of the algorithm, we use an example similar to \cite{garcia-fernandezIteratedStatisticalLinear2014} but alter it to include a dynamical model.
Therefore, let the model be given by
\begin{align*}
\state_{k+1} &\sim \Ndist(\state_{k+1}; a\state_k^3, Q)\\
\obs_k &\sim \Ndist(\obs_k; \state_k, R),
\end{align*}
with $a=0.01, Q=0.1$ and $R=0.1$.
We assume that a prior is given at time $k-1$ as $p(\state_{k-1}|\obs_{1:k-1})=\Ndist(\state_{k-1}; 3, 4)$.
We then apply an extended version of the dynamically iterated filter to this model and plot the intermediary and final approximate predictive, posterior and smoothed densities against a posterior found through a dense numerical grid.
The example is illustrated in \cref{fig:illustrativeexample}, where two iterations are enough for the posterior approximation to be accurate.

\begin{figure}[tb]
\centering\hspace{-.5cm}
\begin{tikzpicture}[every node/.style={inner sep=0pt,outer sep=0pt, font=\footnotesize}]
\node[label=above:{Smoothed / Prior}] (smooth) {\includegraphics[width=.9\columnwidth]{smooth-illustration}};
\node[below= of smooth, label=above:{Predictive}, yshift=.75cm] (pred) {\includegraphics[width=.9\columnwidth]{pred-illustration}};
\node[below= of pred, label=above:{Posterior}, yshift=.75cm] (post) {\includegraphics[width=.9\columnwidth]{post-illustration}};
% \draw[-latex, thick] (smooth.east) to [out=-65, in=65] (pred.east) node[left] {TU};
\draw[-, thick] (smooth.east)++(0,-0.25) edge[-latex, out=-65, in=65] node[left,xshift=-.25cm, yshift=.25cm] {TU} (pred.east);
% \draw[-latex, thick] (pred.east)++(0,-0.25) to [out=-65, in=65] (post.east);
\draw[-, thick] (pred.east)++(0,-0.25) edge[-latex, out=-65, in=65] node[left, xshift=-.25cm, yshift=.25cm] {MU} (post.east);
% \draw[-latex, thick] (post.west) to [out=105, in=-105] (smooth.west);
\draw[-, thick] (post.west) edge[-latex, out=105, in=-105] node[right, xshift=.25cm] {S} (smooth.west);
\end{tikzpicture}
\caption{Illustration of the (extended) dynamically iterated filter.
The black curves in the top and bottom plots are the prior $p(\state_{k-1}|\obs_{1:k-1})$ and true posterior $p(\state_{k}|\obs_{1:k})$, respectively.
The blue curves from top to bottom illustrate the approximate smoothed, predictive and posterior densities at iteration 0, respectively.
The orange curves illustrate the same densities during the second iteration of the filter.
The filter thus moves from the prior (top) to the predictive (middle) to the posterior (bottom) and back up to the smoothed (top).
The time update, measurement update and smoothing step are indicated similarly to \cref{fig:dyniterfilter}.}
\label{fig:illustrativeexample}
\end{figure}
% \begin{figure}[tb]
% \centering
% \includegraphics[width=\columnwidth]{dyniterillustration}
% \caption{Illustration of the (extended) dynamically iterated filter. The prior is illustrated with a dashed black curve whereas the posterior is solid black. The blue colored lines are the first iteration of the filter, whereas the orange colored lines are the second iteration.
% The solid blue and orange lines are the approximate predicted densities (time update). The dashed lines are the approximate posterior densities (measurement update). Lastly, the dotted lines are the approximate smoothed densities.}
% \label{fig:illustrativeexample}
% \end{figure}

